A Survey of Race, Racism, and Anti-Racism in NLP

Despite inextricable ties between race and language, little work has considered race in NLP research and development. In this work, we survey 79 papers from the ACL anthology that mention race. These papers reveal various types of race-related bias in all stages of NLP model development, highlighting the need for proactive consideration of how NLP systems can uphold racial hierarchies. However, persistent gaps in research on race and NLP remain: race has been siloed as a niche topic and remains ignored in many NLP tasks; most work operationalizes race as a fixed single-dimensional variable with a ground-truth label, which risks reinforcing differences produced by historical racism; and the voices of historically marginalized people are nearly absent in NLP literature. By identifying where and how NLP literature has and has not considered race, especially in comparison to related fields, our work calls for inclusion and racial justice in NLP research practices.

==> NLP and Race Survey (1)/notes.tex <==
Reading group notes:
Kartik:
- Section 2 is good: what is race is not discussed in NLP
- Need to clarify what "racialized people" means, might not be clear to NLP people
- ACL community has lots of non-US people. might be useful to talk about what race looks like in different countries; racial bias means different things to different people from different countries. Might resonate with non-US reviewrs more
- Closing statement: talk about HCI and fiarness and ML, might be useful to have a recap of these in the final paragraph and provide some recommendations to people interested in race in NLP. Example, (1) reflexivity in HCI, (2) talk about where you are getting labels from and if they make sense in this context
- Sections that talk about data sources and data sets and places where we don't think about NLP. Should make clear that tagging data with race is not necessarily the best solution (can draw from IBM faces example)
- Output interpretation section: maybe expand this
- Shrink section about how common data sets are narrow in scope
- Kind of striking that no work on power as addressed race

Qinlan:
- not clear what to draw from
- Maybe can consider changing the columns to the other ones
- overall liked it, agree with most of Michael and Kartik's comments. Generally like the message behind it
- Disconnect between how definition of race was introduced and how Alex Hanna paper was cited (make clear what the lessons from this paper should be)
- Might be interesting to look at institutions where papers are from
- Pointing out issue without strong solution could be a critique from reviewers. Even when paper has a weak notion of what to do. Should stress takeaways from each section (rather than grouping at the end)
- People could criticize novelty. Tying together concepts from these papers is the interesting part of the paper. How to tie to papers like Su Lin's or Alex Hanna's might need to be defended

Add Discussions and Conclusions endings that says our goal is to show how this work is relevant to NLP.
Su Lin's paper and other survey's don't look at race

Michael:
- it's a scathing "we don't do this", we draw from HCI is kind of scathing. The "Alternative alternative" ending might be good (or alternate ending, but make clear how examples apply to HCI)
- be up-front about operating under a US-centric conception of race. Maybe add a brief discussion of how race is thought about in other country
- Some discussion about what races are brought up. A lot of it is African American, but not all of it
- Lots of Asian and Asian-American people who do NLP work, that should be somehow acknowledged. Maybe don't want to go deep into that, but a little could work.
- Bringing up context of whiteness as a default thing. Like Ibrham Kendi quote. Thinking about white listening subject
- Might be good to use organization more in Table 1  - show where we do have work. Rows in the table seem a little broad (Some are very broad and some are very specific). Might actually be interesting to break them by NLP tracts
- is there no work on speech? This would be a good thing to point out. Note that we don't want to say there are racial differences in language. We want to say that we've trained our models to find ones
- Underlying issue of the IBM thing, should we really use self-identified race. Maybe in last section point out that data is a problem but that we can't just gather it without talking to the people who own that data

==> NLP and Race Survey (1)/papers.tex <==
\section{Full List of Surveyed Papers}
\label{sec:appendix_papers}

\begin{longtable}{lccccccc}
\hline
 & Year & Venue & NLP Task & Task Type \\
    \hline
    \hline
\footnotesize{\citet{assimakopoulos-etal-2020-annotating}} & 2020 & LREC & Abusive Language & Collect Corpus \\
\footnotesize{\citet{bommasani-etal-2020-interpreting}} & 2020 & ACL & Text Representations & Detect Bias \\
\footnotesize{\citet{chakravarthi-2020-hopeedi}} & 2020 & Workshop & Abusive Language & Collect Corpus \\
\footnotesize{\citet{groenwold-etal-2020-investigating}} & 2020 & EMNLP & Text Generation & Detect Bias \\
\footnotesize{\citet{gupta-etal-2020-heart}} & 2020 & Workshop & Sector-spec. NLP apps. & Collect Corpus \\
\footnotesize{\citet{huang-etal-2020-multilingual}} & 2020 & LREC & Abusive Language & Detect Bias \\
\footnotesize{\citet{jiang-fellbaum-2020-interdependencies}} & 2020 & Workshop & Text Representations & Detect Bias \\
\footnotesize{\citet{joseph-morgan-2020-word}} & 2020 & ACL & Text Representations & Detect Bias \\
\footnotesize{\citet{kennedy-etal-2020-contextualizing}} & 2020 & ACL & Abusive Language & Debias \\
\footnotesize{\citet{kurrek-etal-2020-towards}} & 2020 & Workshop & Abusive Language & Collect Corpus \\
\footnotesize{\citet{lepori-2020-unequal}} & 2020 & COLING & Text Representations & Detect Bias \\
\footnotesize{\citet{liu-etal-2020-gender}} & 2020 & COLING & Text Generation & Debias \\
\footnotesize{\citet{meaney-2020-crossing}} & 2020 & Workshop & Social Science/Media & Survey/Position \\
\footnotesize{\citet{nangia-etal-2020-crows}} & 2020 & EMNLP & Text Representations & Detect Bias \\
\footnotesize{\citet{roy-goldwasser-2020-weakly}} & 2020 & EMNLP & Social Science/Media & Analyze Corpus \\
\footnotesize{\citet{sap-etal-2020-social}} & 2020 & ACL & Abusive Language & Collect Corpus \\
\footnotesize{\citet{shah-etal-2020-predictive}} & 2020 & ACL & Ethics/Task-indep. Bias & Survey/Position \\
\footnotesize{\citet{shahid-etal-2020-detecting}} & 2020 & Workshop & Social Science/Media & Analyze Corpus \\
\footnotesize{\citet{tan-etal-2020-morphin}} & 2020 & ACL & Ethics/Task-indep. Bias & Develop Model \\
\footnotesize{\citet{xia-etal-2020-demoting}} & 2020 & Workshop & Abusive Language & Debias \\
\footnotesize{\citet{zhang-etal-2020-demographics}} & 2020 & ACL & Abusive Language & Detect Bias \\
\footnotesize{\citet{zhao-chang-2020-logan}} & 2020 & EMNLP & Ethics/Task-indep. Bias & Detect Bias \\
\footnotesize{\citet{amir-etal-2019-mental}} & 2019 & Workshop & Sector-spec. NLP apps. & Analyze Corpus \\
\footnotesize{\citet{davidson-etal-2019-racial}} & 2019 & Workshop & Abusive Language & Detect Bias \\
\footnotesize{\citet{demszky-etal-2019-analyzing}} & 2019 & NAACL & Social Science/Media & Analyze Corpus \\
\footnotesize{\citet{gillani-levy-2019-simple}} & 2019 & Workshop & Text Representations & Analyze Corpus \\
\footnotesize{\citet{jurgens-etal-2019-just}} & 2019 & ACL & Abusive Language & Survey/Position \\
\footnotesize{\citet{karve-etal-2019-conceptor}} & 2019 & Workshop & Text Representations & Debias \\
\footnotesize{\citet{kurita-etal-2019-measuring}} & 2019 & Workshop & Text Representations & Detect Bias \\
\footnotesize{\citet{lauscher-glavas-2019-consistently}} & 2019 & Workshop & Text Representations & Detect Bias \\
\footnotesize{\citet{lee-etal-2019-exploring}} & 2019 & Workshop & Text Generation & Detect Bias \\
\footnotesize{\citet{liu-etal-2019-detecting}} & 2019 & CoNLL & Social Science/Media & Develop Model \\
\footnotesize{\citet{manzini-etal-2019-black}} & 2019 & NAACL & Text Representations & Debias \\
\footnotesize{\citet{may-etal-2019-measuring}} & 2019 & ACL & Text Representations & Detect Bias \\
\footnotesize{\citet{mayfield-etal-2019-equity}} & 2019 & Workshop & Sector-spec. NLP apps. & Survey/Position \\
\footnotesize{\citet{merullo-etal-2019-investigating}} & 2019 & EMNLP & Social Science/Media & Analyze Corpus \\
\footnotesize{\citet{mostafazadeh-davani-etal-2019-reporting}} & 2019 & EMNLP & Core NLP Applications & Develop Model \\
\footnotesize{\citet{parish-morris-2019-computational}} & 2019 & Workshop & Sector-spec. NLP apps. & Survey/Position \\
\footnotesize{\citet{romanov-etal-2019-whats}} & 2019 & NAACL & Sector-spec. NLP apps. & Debias \\
\footnotesize{\citet{santos-paraboni-2019-moral}} & 2019 & RANLP & Social Science/Media & Collect Corpus \\
\footnotesize{\citet{sap-etal-2019-risk}} & 2019 & ACL & Abusive Language & Detect Bias \\
\footnotesize{\citet{sharifirad-matwin-2019-using}} & 2019 & Workshop & Abusive Language & Analyze Corpus \\
\footnotesize{\citet{sommerauer-fokkens-2019-conceptual}} & 2019 & Workshop & Text Representations & Detect Bias \\
\footnotesize{\citet{tripodi-etal-2019-tracing}} & 2019 & Workshop & Text Representations & Analyze Corpus \\
\footnotesize{\citet{vylomova-etal-2019-evaluation}} & 2019 & Workshop & Social Science/Media & Analyze Corpus \\
\footnotesize{\citet{wallace-etal-2019-universal}} & 2019 & EMNLP & Text Generation & Detect Bias \\
\footnotesize{\citet{xu-etal-2019-privacy}} & 2019 & INLG & Text Generation & Develop Model \\
\footnotesize{\citet{barbieri-camacho-collados-2018-gender}} & 2018 & *SEM & Social Science/Media & Analyze Corpus \\
\footnotesize{\citet{blodgett-etal-2018-twitter}} & 2018 & ACL & Core NLP Applications & Debias \\
\footnotesize{\citet{castelle-2018-linguistic}} & 2018 & Workshop & Abusive Language & Analyze Corpus \\
\footnotesize{\citet{de-gibert-etal-2018-hate}} & 2018 & Workshop & Abusive Language & Collect Corpus \\
\footnotesize{\citet{elazar-goldberg-2018-adversarial}} & 2018 & EMNLP & Ethics/Task-indep. Bias & Debias \\
\footnotesize{\citet{kasunic-kaufman-2018-learning}} & 2018 & Workshop & Text Generation & Survey/Position \\
\footnotesize{\citet{kiritchenko-mohammad-2018-examining}} & 2018 & *SEM & Social Science/Media & Detect Bias \\
\footnotesize{\citet{loveys-etal-2018-cross}} & 2018 & Workshop & Sector-spec. NLP apps. & Analyze Corpus \\
\footnotesize{\citet{preotiuc-pietro-ungar-2018-user}} & 2018 & COLING & Social Science/Media & Develop Model \\
\footnotesize{\citet{sheng-etal-2019-woman}} & 2018 & EMNLP & Text Generation & Detect Bias \\
\footnotesize{\citet{wojatzki-etal-2018-quantifying}} & 2018 & LREC & Social Science/Media & Collect Corpus \\
\footnotesize{\citet{wood-doughty-etal-2018-predicting}} & 2018 & Workshop & Social Science/Media & Develop Model \\
\footnotesize{\citet{clarke-grieve-2017-dimensions}} & 2017 & Workshop & Abusive Language & Analyze Corpus \\
\footnotesize{\citet{gallagher-etal-2017-anchored}} & 2017 & TACL & Social Science/Media & Develop Model \\
\footnotesize{\citet{hasanuzzaman-etal-2017-demographic}} & 2017 & IJCNLP & Abusive Language & Develop Model \\
\footnotesize{\citet{ramakrishna-etal-2017-linguistic}} & 2017 & ACL & Social Science/Media & Analyze Corpus \\
\footnotesize{\citet{rudinger-etal-2017-social}} & 2017 & Workshop & Core NLP Applications & Detect Bias \\
\footnotesize{\citet{schnoebelen-2017-goal}} & 2017 & Workshop & Ethics/Task-indep. Bias & Survey/Position \\
\footnotesize{\citet{van-miltenburg-etal-2017-cross}} & 2017 & INLG & Image Processing & Detect Bias \\
\footnotesize{\citet{waseem-etal-2017-understanding}} & 2017 & Workshop & Abusive Language & Survey/Position \\
\footnotesize{\citet{wood-doughty-etal-2017-twitter}} & 2017 & Workshop & Social Science/Media & Analyze Corpus \\
\footnotesize{\citet{wright-etal-2017-vectors}} & 2017 & Workshop & Abusive Language & Analyze Corpus \\
\footnotesize{\citet{blodgett-etal-2016-demographic}} & 2016 & EMNLP & Ethics/Task-indep. Bias & Collect Corpus \\
\footnotesize{\citet{pavlick-etal-2016-gun}} & 2016 & EMNLP & Core NLP Applications & Collect Corpus \\
\footnotesize{\citet{waseem-2016-racist}} & 2016 & Workshop & Abusive Language & Detect Bias \\
\footnotesize{\citet{waseem-hovy-2016-hateful}} & 2016 & Workshop & Abusive Language & Collect Corpus \\
\footnotesize{\citet{mohammady-culotta-2014-using}} & 2014 & Workshop & Social Science/Media & Develop Model \\
\footnotesize{\citet{bergsma-etal-2013-broadly}} & 2013 & NAACL & Social Science/Media & Develop Model \\
\footnotesize{\citet{herbelot-etal-2012-distributional}} & 2012 & Workshop & Social Science/Media & Analyze Corpus \\
\footnotesize{\citet{warner-hirschberg-2012-detecting}} & 2012 & Workshop & Abusive Language & Develop Model \\
\footnotesize{\citet{eisenstein-etal-2011-discovering}} & 2011 & ACL & Social Science/Media & Analyze Corpus \\
\footnotesize{\citet{somers-2006-language}} & 2006 & Workshop & Sector-spec. NLP apps. & Survey/Position \\
\end{longtable}

==> notes.tex <==
Reading group notes:
Kartik:
- Section 2 is good: what is race is not discussed in NLP
- Need to clarify what "racialized people" means, might not be clear to NLP people
- ACL community has lots of non-US people. might be useful to talk about what race looks like in different countries; racial bias means different things to different people from different countries. Might resonate with non-US reviewrs more
- Closing statement: talk about HCI and fiarness and ML, might be useful to have a recap of these in the final paragraph and provide some recommendations to people interested in race in NLP. Example, (1) reflexivity in HCI, (2) talk about where you are getting labels from and if they make sense in this context
- Sections that talk about data sources and data sets and places where we don't think about NLP. Should make clear that tagging data with race is not necessarily the best solution (can draw from IBM faces example)
- Output interpretation section: maybe expand this
- Shrink section about how common data sets are narrow in scope
- Kind of striking that no work on power as addressed race

Qinlan:
- not clear what to draw from
- Maybe can consider changing the columns to the other ones
- overall liked it, agree with most of Michael and Kartik's comments. Generally like the message behind it
- Disconnect between how definition of race was introduced and how Alex Hanna paper was cited (make clear what the lessons from this paper should be)
- Might be interesting to look at institutions where papers are from
- Pointing out issue without strong solution could be a critique from reviewers. Even when paper has a weak notion of what to do. Should stress takeaways from each section (rather than grouping at the end)
- People could criticize novelty. Tying together concepts from these papers is the interesting part of the paper. How to tie to papers like Su Lin's or Alex Hanna's might need to be defended

Add Discussions and Conclusions endings that says our goal is to show how this work is relevant to NLP.
Su Lin's paper and other survey's don't look at race

Michael:
- it's a scathing "we don't do this", we draw from HCI is kind of scathing. The "Alternative alternative" ending might be good (or alternate ending, but make clear how examples apply to HCI)
- be up-front about operating under a US-centric conception of race. Maybe add a brief discussion of how race is thought about in other country
- Some discussion about what races are brought up. A lot of it is African American, but not all of it
- Lots of Asian and Asian-American people who do NLP work, that should be somehow acknowledged. Maybe don't want to go deep into that, but a little could work.
- Bringing up context of whiteness as a default thing. Like Ibrham Kendi quote. Thinking about white listening subject
- Might be good to use organization more in Table 1  - show where we do have work. Rows in the table seem a little broad (Some are very broad and some are very specific). Might actually be interesting to break them by NLP tracts
- is there no work on speech? This would be a good thing to point out. Note that we don't want to say there are racial differences in language. We want to say that we've trained our models to find ones
- Underlying issue of the IBM thing, should we really use self-identified race. Maybe in last section point out that data is a problem but that we can't just gather it without talking to the people who own that data
